A Redshifted Inner Disk Atmosphere and Transient Absorbers in the Ultra-Compact Neutron Star X-ray Binary 4U 1916-053

The very small accretion disks in ultra-compact X-ray binaries (UCXBs) are special laboratories in which to study disk accretion and outflows. We report on three sets of new (250 ks total) and archival (50 ks) Chandra/HETG observations of the "dipping" neutron-star X-ray binary 4U 1916$-$053, which has an orbital period of $P\simeq 50$~minutes. We find that the bulk of the absorption in all three spectra originates in a disk atmosphere that is redshifted by $v\simeq 220-290$ $\text{km}$ $\text{s}^{-1}$, corresponding to the gravitational redshift at radius of $R \sim 1200$ $GM/{c}^{2}$. This shift is present in the strongest, most highly ionized lines (Si XIV and Fe XXVI), with a significance of 5$\sigma$. Absorption lines observed during dipping events (typically associated with the outermost disk) instead display no velocity shifts and serve as a local standard of rest, suggesting that the redshift is intrinsic to an inner disk atmosphere and not due to radial motion in the galaxy or a kick. In two spectra, there is also evidence of a more strongly redshifted component that would correspond to a disk atmosphere at $R \sim 70$ $GM/{c}^{2}$; this component is significant at the 3$\sigma$ level. Finally, in one spectrum, we find evidence of disk wind with a blue shift of $v = {-1700}^{+1700}_{-1200}$ $\text{km}$ $\text{s}^{-1}$. If real, this wind would require magnetic driving.

==> table3.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.23}
\caption{Wind Parameters for Spectrum A}
\vspace{-1.0\baselineskip}
\begin{footnotesize}
\begin{center}
\begin{tabular*}{0.47\textwidth}{l @{\extracolsep{\fill}} c c}
\tableline
\tableline


Method  & $R = {R}_{Upper}$&$R = {R}_{Orbital}$  \\
& ($R \leq L/{N}_{He}\xi$)&($R = G M/{\sigma}_{emis}^{2}$) \\
\tableline 
${R}_{Launch}$ (${10}^{8}$ cm)&
$\leq{13}^{+7}_{-8}$ & 
${7.2}^{+1.5}_{-1.7}$\\

${R}_{Launch}$ $(GM/{c}^{2}$) &
$\leq{8500}^{+4600}_{-5500}$ & 
${4800}^{+1000}_{-1100}$ \\

${R}_{Launch}/0.1{R}_{C}$ & 
$\leq{0.15} \pm 0.1$ &
${0.09} \pm 0.02$  \\

${n}_{He}$ (${10}^{14}$ ${cm}^{-3}$)& 
$\geq{0.8} \pm 0.5$ & 
${2.5} \pm 0.8$  \\

$f$&
$\leq{1.0}^{\dagger}$& 
${0.6}^{+0.4}_{-0.3}$ \\

$\dot{M}_{wind}$ (${10}^{16}$ g/s)&
$\leq{7.1}^{+2.8}_{-2.4}$ & ${4.3}^{+1.7}_{-1.5}$ \\


$\dot{M}_{wind}$/$\dot{M}_{in}$ & 
$\leq{0.8}^{+0.3}_{-0.2}$ & 
${0.5}^{+0.2}_{-0.2}$ \\


${L}_{wind}$ (${10}^{32}$ erg/s)& 
$\leq{10}^{+7}_{-5}$ & 
${6}^{+4}_{-3}$ \\


${L}_{wind}$/${L}_{rad}$ (${10}^{-4}$)&
$\leq{15}^{+8}_{-6}$ &
${9.1}^{+4.9}_{-3.9}$ \\ 




\\ [-3.0ex]
\tableline 
\tableline 


\end{tabular*}
\vspace*{-1.0\baselineskip}~\\ \end{center} 
\tablecomments{Physical parameters of the wind found in Spectrum A, derived using the best-fit model parameters listed in Table \ref{tab:fit}. The first column lists the properties of the wind using the upper limit on the photoionization radius ${R}_{launch} = f\cdot{R}_{upper}$ assuming a filling factor of unity, where $R \leq {R}_{upper} \equiv L/{N}_{He}\xi$. Values listed on the first column are therefore either upper or lower limits. Values in the second column are calculated using the orbital radius ${R}_{launch} =  {R}_{orbital}$, where we treated best-fit velocity broadening of wind re-emission lines as representative of the local Keplerian velocity. Although neutron star mass of $1{M}_{\odot}$ was assumed, a mass of $\sim 1.7{M}_{\odot}$ would result in a filling factor of unity, and the values in the second column would match those in the first (which, for the most part, are mass-independent). See text for details. }
\end{footnotesize}
\label{tab:wind}
\end{table}
